Edge-based fever screening system over private 5G

Edge computing and 5G have made it possible to perform analytics closer to the source of data and achieve super-low latency response times, which is not possible with centralized cloud deployment. In this paper, we present a novel fever-screening system, which uses edge machine learning techniques and leverages private 5G to accurately identify and screen individuals with fever in real-time. Particularly, we present deep-learning based novel techniques for fusion and alignment of cross-spectral visual and thermal data streams at the edge. Our novel Cross-Spectral Generative Adversarial Network (CS-GAN) synthesizes visual images that have the key, representative object level features required to uniquely associate objects across visual and thermal spectrum. Two key features of CS-GAN are a novel, feature-preserving loss function that results in high-quality pairing of corresponding cross-spectral objects, and dual bottleneck residual layers with skip connections (a new, network enhancement) to not only accelerate real-time inference, but to also speed up convergence during model training at the edge. To the best of our knowledge, this is the first technique that leverages 5G networks and limited edge resources to enable real-time feature-level association of objects in visual and thermal streams (30 ms per full HD frame on an Intel Core i7-8650 4-core, 1.9GHz mobile processor). To the best of our knowledge, this is also the first system to achieve real-time operation, which has enabled fever screening of employees and guests in arenas, theme parks, airports and other critical facilities. By leveraging edge computing and 5G, our fever screening system is able to achieve 98.5% accuracy and is able to process about 5X more people when compared to a centralized cloud deployment.

==> files/applications.tex <==
\section{Application}
\subsection{Thermal screening system}
Our proposed cross-spectral object association and depth estimation is a key component of an application that simultaneously performs face-based authentication, and fever screening for employees and guests. It can also be used for other applications like  non-contact vital sign monitoring, non-contact-rgb-infrared, emotion recognition, and biometric authentication. 

%It can also be used for other applications like  non-contact vital sign monitoring \cite{non-contact-vital-sign, non-contact-rgb-infrared}, emotion recognition \cite{emotion-recognition}, and biometric authentication \cite{biometric-authentication}.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.65\linewidth]{images/depth-perception.png}
    \vskip -0.1in
    \caption{Elevated body temperature screening}
    \lFig{depth-perception}
\end{figure}
\vskip -0.1in
%where fusion of different sensor modalities is required. As an illustration of our technique, we have shown fusion of thermal and visual data streams in real-time to obtain association between objects and estimate their depth. This is required in several real-time applications like non-contact vital sign monitoring \cite{non-contact-vital-sign, non-contact-rgb-infrared}, emotion recognition \cite{emotion-recognition}, biometric authentication \cite{biometric-authentication}, etc. 
%Using our system as a core building block, we implemented a real-time application which simultaneously allows us to perform face-based authentication, as well as screen for people with elevated body temperature. 

%We designed a novel real-time application that simultaneously performs face-based authentication, and elevated body temperature screening for employees and guests.  

As shown in \rFig{depth-perception}, thermal and visual cameras monitor a particular area. 
%These cameras are co-located next to each other and have slightly different field of view. 
%As people walk by, we authenticate them by using face-recognition, and screen them for elevated body temperature, in real-time. 
For non-invasive febrile temperature screening, ISO recommends a temperature measurement at the inner canthus of the eyes where the temperature is close to the core body temperature \cite{ISO/TR13154:2017}. However, detecting this region using just thermal data is inaccurate \cite{face-landmark-on-thermal}. We use our cross-spectral association to accurately locate the inner canthus in the thermal data by first locating it in the visual stream by using a face detection engine. 
%visual stream where detection accuracy is high \cite{facial-landmark-on-rgb}, but due to displacement between cameras, there is misalignment, and accurately mapping eye region in visual stream to corresponding region in thermal stream (to measure temperature) is a challenge. 
The measured temperature also depends on the distance from the sensors \cite{variation-in-temperature}. 
%This variation in temperature based on distance becomes another challenge and requires appropriate temperature correction. 
So, our system detects faces and estimates their depth in real-time. Overall, our system (a) authenticates people, (b) measures their core body temperature, (c) corrects measured temperature based on the distance from the sensors, and finally (d) screens those with elevated body temperature. 
%Right side of \rFig{depth-perception} shows liveliness check for individuals (Real/Fake), their measured distances (at bottom of pictures) and also screening those with elevated body temperature (marked with Fever). 
This application is currently deployed (field trials) at several customer sites (casinos, arenas, theme parks, and airports).

\subsection{Evaluation of performance on Edge vs Cloud}

Key metric in thermal screening system is to receive fever alerts in real-time, so that persons can enter the facility without having to wait to be screened. In the proposed free-flow screening system, as people are moving in their natural walking pace, we often have only under 100ms per frame to be processed and insights to be generated. We compared our system with two different implementations.

First one is fully cloud based approach, where the AI modules are running in the cloud and all sensor traffic is routed to the cloud. Often the round-trip latency for communicating to cloud is in the order of 100's of milliseconds. With the computation time as discussed in \rSec{result-quantitative-analysis} being around 50ms, total latency for alert is greater than 250ms which is unsuitable for real-time application.

Second is the approach we used based on Edge computing technology where MEC (Multi-access Edge Computing) servers at cellular edge, processes heavy computation loads which the AI algorithms demand. Round trip latency to local edge server is in the order of sub-milliseconds. Including computation time, total turnaround time for an alert is less than 75ms which is suitable for free flow screening application.

